Automated reasoning support for Standpoint-OWL 2

We present a tool for modelling and reasoning with knowledge from various diverse (and possibly conflicting) viewpoints. The theoretical underpinnings are provided by enhancing base logics by standpoints according to a recently introduced formalism that we also recall. The tool works by translating the standpoint-enhanced version of the description logic SROIQ to its plain (i.e. classical) version. Existing reasoners can then be directly used to provide automated support for reasoning about diverse standpoints.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> Text/Acknowledgments.tex <==
\todo{TODO.}

==> macros/davidMacros.tex <==
%% Preamble
% \usepackage{amsmath}
% % Commands: \eqref
% \usepackage{amssymb}
% % Commands: \square
% \usepackage{enumitem}
% \setlist[itemize]{leftmargin=*}
% \setlist[enumerate]{leftmargin=*}
% %
% \usepackage{geometry}
% \geometry{left=20mm, top=20mm, right=60mm, textwidth=20mm}
% %
% \usepackage{hyperref}
% % Commands: \href
% \usepackage{mathbbol}
% % Enables the use of lowercase \mathbb characters
% \usepackage[framemethod=tikz]{mdframed}
% % Commands: \newmdtheoremenv
% \usepackage[numbers]{natbib}
% % Commands: \citeauthor
% \usepackage{luatodonotes}
% % Commands: \todo
% \usepackage{xspace}
% % Commands: \xspace
% \usetikzlibrary{arrows.meta}
% % \path[-{Latex[length=5mm, width=2mm]}]
% \pagenumbering{gobble}


% %% Environments
% \newenvironment{proof}{\vspace{-0.75cm}\paragraph{Proof:}}{\hfill$\square$\vspace{0.25cm}}
% \newmdtheoremenv[backgroundcolor=none]{BoxCorollary}{Corollary}[subsection]
% \newmdtheoremenv[backgroundcolor=none]{BoxDefinition}{Definition}[subsection]
% \newmdtheoremenv[backgroundcolor=none]{BoxDiscussion}{Non-Essential Discussion}[subsection]
% \newmdtheoremenv[backgroundcolor=none]{BoxRemark}{Remark}[subsection]
% %\newmdtheoremenv[tikzsetting={draw=black,fill=gray,fill opacity=0.05}]{BoxDiscussion}{Discussion}[subsection]
% \newmdtheoremenv[backgroundcolor=none]{BoxExample}{Example}[subsection]
% \newmdtheoremenv[backgroundcolor=none]{BoxLemma}{Lemma}[subsection]
% \newmdtheoremenv[backgroundcolor=none]{BoxProof}{Theorem}[subsection]
% \newmdtheoremenv[backgroundcolor=none]{BoxProposition}{Proposition}[subsection]
% \newmdtheoremenv[backgroundcolor=none]{BoxTheorem}{Theorem}[subsection]

% Todos
\newcommand{\TodoFormat}[1]{\footnotesize{#1}}
\newcommand{\Todo}[1]{\todo[linecolor=black!20, backgroundcolor=white, bordercolor=black, leaderwidth=1pt]{\TodoFormat{#1}}}
%\newcommand{\Todo}[1]{\todo[linecolor=green!70!white,leaderwidth=5pt,color=gray!10]{\TodoFormat{#1}}}
% Font Formatting
\newcommand{\FormatArithmeticComplexityClass}[1]{\ensuremath{\textsc{#1}}\xspace}
\newcommand{\FACC}[1]{\FormatArithmeticComplexityClass{#1}}
\newcommand{\FormatEntitySet}[1]{\ensuremath{\mathsf{#1}}\xspace}
\newcommand{\FormatFormulaSet}[1]{\ensuremath{\mathcal{#1}}\xspace}
\newcommand{\FormatFormulaSetOfSets}[1]{\ensuremath{\mathfrak{#1}}\xspace}
\newcommand{\FormatFunction}[1]{\ensuremath{\mathbb{#1}}\xspace}
\newcommand{\FF}[1]{\FormatFunction{#1}}
\newcommand{\FormatLanguage}[1]{\ensuremath{\mathsf{#1}}\xspace}
\newcommand{\FL}[1]{\FormatLanguage{#1}}
\newcommand{\FormatPredicate}[1]{\ensuremath{\mathtt{#1}}\xspace}
\newcommand{\FP}[1]{\FormatPredicate{#1}}
\newcommand{\FormatTM}[1]{\ensuremath{\mathit{#1}}\xspace}
% Sets of Numbers
\newcommand{\NaturalNumbers}{\ensuremath{\FormatSetOfNumbers{N}}\xspace}
\newcommand{\PositiveIntegers}{\ensuremath{\FormatSetOfNumbers{N}_{>0}}\xspace}
% Items
\newcommand{\FirstItem}{(i)\xspace}
\newcommand{\SecondItem}{(ii)\xspace}
\newcommand{\ThirdItem}{(iii)\xspace}
\newcommand{\FourthItem}{(iv)\xspace}
\newcommand{\FifthItem}{(v)\xspace}
% Complexity and Arithmetic Classes of Languages
\newcommand{\ComplexityClass}{\FACC{c}}
\newcommand{\PTime}{\FormatArithmeticComplexityClass{P}}
\newcommand{\NP}{\FormatArithmeticComplexityClass{NP}}
\newcommand{\LogSpace}{\FormatArithmeticComplexityClass{LogSpace}}
\newcommand{\PSpace}{\FormatArithmeticComplexityClass{PSpace}}
\newcommand{\ExpTime}{\FormatArithmeticComplexityClass{ExpTime}}
\newcommand{\NExpTime}{\FormatArithmeticComplexityClass{NExpTime}}
\newcommand{\DoubleExpTime}{\FormatArithmeticComplexityClass{2ExpTime}}
\newcommand{\NExpExpTime}{\FormatArithmeticComplexityClass{N2ExpTime}}
\newcommand{\RecursivelEnumerable}{\FormatArithmeticComplexityClass{Re}}
\newcommand{\RE}{\RecursivelEnumerable}
\newcommand{\CoArithmeticClass}[1]{\ensuremath{\Pi^0_{#1}}\xspace}
\newcommand{\CAC}[1]{\CoArithmeticClass{#1}}


==> macros/dlmacros.tex <==

\newcommand{\Domain}{\Delta}
\newcommand{\conceptdom}{\top}

%\newcommand{\define}[1]{\textsc{#1}}
%\newcommand{\define}[1]{\emph{#1}}
%\newcommand{\tuple}[1]{\langle{#1}\rangle}

\hyphenation{equi-sat-is-fi-able} % prevent "eq-ui"

%%% Various DLs
%\newcommand{\HornSHIQ}{Horn-$\mathcal{SHIQ}$}
%\newcommand{\HornFLE}{Horn-$\mathcal{F\!\!LE}$}
%\newcommand{\DLmin}{\ensuremath{\text{DL}_{\mathsf{min}}}\xspace}
\newcommand{\DLmin}{\ensuremath{\mathsf{DL_{min}}}\xspace}
\newcommand{\DLite}{DL-Lite\xspace}
\newcommand{\DLitec}{\ensuremath{\mathsf{DL}\text{-Lite}_{\mathsf{core}}}\xspace}
\newcommand{\SROIQ}{\ensuremath{\mathcal{SROIQ}}\xspace}
\newcommand{\SROIQbs}{\ensuremath{\mathcal{SROIQ}b_s}\xspace}
\newcommand{\SROIQK}{$\mathcal{SROIQK}$}
\newcommand{\SRIQ}{$\mathcal{SRIQ}$}
\newcommand{\SHOIQ}{$\mathcal{SHOIQ}$}
\newcommand{\SHOIN}{$\mathcal{SHOIN}$}
\newcommand{\SHIQ}{$\mathcal{SHIQ}$}
\newcommand{\SHOQ}{$\mathcal{SHOQ}$}
\newcommand{\SHOI}{$\mathcal{SHOI}$}
%\newcommand{\SHIQB}{$\mathcal{SHIQB}$}
% \newcommand{\SHIQb}{$\mathcal{SHIQ}b$}
\newcommand{\ALC}{$\mathcal{ALC}$}
% \newcommand{\FLE}{$\mathcal{F\!\!LE}$}
%\newcommand{\EL}{$\mathcal{EL}$}
\newcommand{\ELpp}{$\mathcal{EL}^{\mathord{+}\mathord{+}}$}
\newcommand{\ELRO}{$\mathcal{ELRO}$}
\newcommand{\ALCHIQ}{$\mathcal{ALCHIQ}$}
\newcommand{\ALCHOI}{$\mathcal{ALCHOI}$}
\newcommand{\ALCHIqb}{$\mathcal{ALCHI}b^{\le}$}
\newcommand{\ALCIqb}{$\mathcal{ALCI}b^{\le}$}
\newcommand{\ALCIFb}{$\mathcal{ALCIF}b$}
\newcommand{\ALCIb}{$\mathcal{ALCI}b$}
%% extended with concept product:
\newcommand{\ALCHOIX}{$\mathcal{ALCHOI}^{\times}$}
\newcommand{\ALCHOIQX}{$\mathcal{ALCHOIQ}^{\times}$}
\newcommand{\SROIQX}{$\mathcal{SROIQ}^{\times}$}
\newcommand{\SHOIQX}{$\mathcal{SHOIQ}^{\times}$}
\newcommand{\SHIQX}{$\mathcal{SHIQ}^{\times}$}
% \newcommand{\SHIQx}{$\mathcal{SHIQ}^{(\times)}$}
\newcommand{\SHOQX}{$\mathcal{SHOQ}^{\times}$}
\newcommand{\SHOIX}{$\mathcal{SHOI}^{\times}$}
\newcommand{\ELROX}{$\mathcal{ELRO}^{\times}$}
\newcommand{\ELppX}{$\mathcal{EL}^{\mathord{+}\mathord{+}\mathord{\times}}$}
%% extended with DL rules (tentative) -- removed, we just need role bases anyway
% \newcommand{\ELppR}{$r\mathcal{EL}^{\mathord{+}\mathord{+}}$}

%
\newcommand{\csps}{constraint satisfaction problems\xspace}
\newcommand{\csp}{constraint satisfaction problem\xspace}
\newcommand{\CSPs}{CSPs\xspace}
\newcommand{\CSP}{CSP\xspace}


% COMPLEXITY CLASS
%\newcommand{\NP}{\mbox{\sc{NP}}\xspace}
\newcommand{\NPc}{\mbox{\sc{NP}}-complete\xspace}
\newcommand{\NPh}{\mbox{\sc{NP}}-hard\xspace}
\newcommand{\NPhness}{\mbox{\sc{NP}}-hardness\xspace}
%\newcommand{\ExpTime}{\mbox{\sc{ExpTime}}\xspace}
\newcommand{\TwoExpTime}{\mbox{\sc{2\ExpTime}}\xspace}
\newcommand{\NTwoExpTime}{\mbox{\sc{N\TwoExpTime}}\xspace}
\newcommand{\coNP}{\mbox{\sc{co\NP}}\xspace}

%%% Complexity classes
%\hyphenation{Exp-Time} % prevent "Ex-PTime" (see, e.g. Tobies'01, Glimm'07 ;-)
%\hyphenation{NExp-Time} % better that than something else
%\newcommand{\PSpace}{{\mbox{\sc{PSpace}}}\xspace}
\newcommand{\NPSpace}{{\mbox{\sc{NPSpace}}}\xspace}
\newcommand{\NLogSpace}{{\sc{NLogSpace}}}
%\newcommand{\LogSpace}{{\sc{LogSpace}}\xspace}
%\newcommand{\NP}{{\sc{NP}}}
%\newcommand{\PTime}{\mbox{\sc{P}}\xspace}
%\newcommand{\ExpTime}{{\sc{ExpTime}}}
%\newcommand{\NExpTime}{{\sc{NExpTime}}}

% PROBLEMS
\newcommand{\SAT}{\ensuremath{\mathsf{SAT}}\xspace}
\newcommand{\SATbm}{\ensuremath{\mathsf{SAT_{bm}}\xspace}}


%%% Interpretations & truth values
\newcommand{\Inter}{\mathcal{I}} %used to denote an interpretation
\newcommand{\Jnter}{\mathcal{J}} %used to denote another interpretation
\newcommand{\Knter}{\mathcal{K}} %used to denote yet another interpretation
\newcommand{\true}{\mathit{true}}
\newcommand{\false}{\mathit{false}}

%%% The generic quantor
\RequirePackage{graphicx}
\newcommand{\quantor}{\mathord{\reflectbox{$\text{\sf{Q}}$}}}

%%% DL syntax
\newcommand{\kb}{\text{\rm{KB}}} % the generic knowledge base
\newcommand{\rb}{\text{\rm{RB}}} % the generic rule base
\newcommand{\Ind}[1]{\ensuremath{\mathsf{Ind}(#1)}\xspace}
\newcommand{\lang}[1]{\ensuremath{\mathbf{#1}}} % any "language" name
\newcommand{\rolnames}{{\text{\sf{N}}_R}} % the set of all role names
\newcommand{\connames}{{\text{\sf{N}}_C}} % the set of all concept names
\newcommand{\indnames}{{\text{\sf{N}}_I}} % the set of all individual names
\newcommand{\Vlang}{\ensuremath{\mathbf{V}}} % the set of all variables
\newcommand{\Rlang}{\ensuremath{\mathbf{R}}} % the set of all role names + inverses
\newcommand{\Clang}{\ensuremath{\mathbf{C}}} % the set of all concept names
%\newcommand{\Ilang}{\ensuremath{\mathbf{I}}} % the set of all individual names
%\newcommand{\Vlang}{\ensuremath{\mathbf{V}}} % the set of all variable names
\newcommand{\Var}{\text{\sf{Var}}} % function for mapping queries to sets of variables

\newcommand{\ssb}{\sqsubseteq}
\newcommand{\atleast}[1]{\mathord{\geqslant}#1\,}
\newcommand{\atmost}[1]{\mathord{\leqslant}#1\,}
\newcommand{\cprod}{\times}

% use standard serif/it math font
\newcommand{\conc}[1]{#1}
\newcommand{\rol}[1]{#1}
\newcommand{\ind}[1]{#1}
\newcommand{\inda}{\ind{a}}
\newcommand{\indb}{\ind{b}}
\newcommand{\indc}{\ind{c}}
\newcommand{\indd}{\ind{d}}
\newcommand{\rolexpR}{\rol{r}}
\newcommand{\rolexpS}{\rol{s}}
\newcommand{\rolR}{\mathtt{r}}
\newcommand{\rolS}{\mathtt{s}}
\newcommand{\rolT}{\mathtt{t}}
\newcommand{\rolU}{\mathtt{u}}
\newcommand{\rolV}{\rol{V}}
\newcommand{\rolW}{\rol{W}}
\newcommand{\conA}{\mathtt{A}}
\newcommand{\conB}{\mathtt{B}}
\newcommand{\conC}{\conc{C}}
\newcommand{\conD}{\conc{D}}
\newcommand{\conE}{\conc{E}}
\newcommand{\conF}{\conc{F}}
\newcommand{\conS}{\mathtt{M}}

\newcommand{\roleaxiom}[1]{\text{\sf{#1}}} % used fo Rbox axioms
%\newcommand{\Tra}{\roleaxiom{Tra}} % transitivity axioms (Rbox)
%\newcommand{\Sym}{\roleaxiom{Sym}} % symmetry axioms (Rbox)
%\newcommand{\Asy}{\roleaxiom{Asy}} % asymmetry axioms (Rbox)
%\newcommand{\Dis}{\roleaxiom{Dis}} % disjointness axioms (Rbox)
%\newcommand{\Ref}{\roleaxiom{Ref}} % reflexivity axioms (Rbox)
%\newcommand{\Irr}{\roleaxiom{Irr}} % irreflexivity axioms (Rbox)
%\newcommand{\Self}{\text{\sf{Self}}} % "Self" pseudo-concept
%\newcommand{\Inv}{\text{\rm{Inv}}} % inverted role

%\newcommand{\Trans}{\text{\sf{Trans}}}
\newcommand{\Sing}{\text{\sf{Sing}}}

%%% Knowledge base transformations:
\newcommand{\Epsilon}{\Theta}
\newcommand{\NNF}{\text{\sf{NNF}}} % negation normal form
\newcommand{\FLAT}{\text{{\sf FLAT}}} % "flattening"
\newcommand{\Es}{\Epsilon_{\mathcal{S}}} % eliminate transitivity
\newcommand{\Ege}{\Epsilon_{\ge}} % eliminate atleast
\newcommand{\Eh}{\Epsilon_{\mathcal{H}}} % eliminate role hierarchy
\newcommand{\Ele}{\Epsilon_{\le}} % eliminate atmost
\newcommand{\Ef}{\Epsilon_{\mathcal{F}}} % eliminate functional roles
\newcommand{\clos}{\text{\sf{clos}}} % whatever

% GENERAL
\newcommand{\wrt}{w.r.t.\ }
\newcommand{\ifft}{iff\xspace}
\newcommand{\ie}{i.e.\ }
\newcommand{\eg}{e.g.\ }
\newcommand{\etal}{et\,al.\ }
\newcommand{\cf}{cf.\ }

\newcommand{\Naive}{Na\"ive\xspace}
\newcommand{\naive}{na\"ive\xspace}

% Semantic Web
\newcommand{\OWL}{OWL\xspace}
\newcommand{\OWLTwo}{OWL\,2\xspace}
\newcommand{\OWLDL}{OWL-DL\xspace}
\newcommand{\API}{API\xspace}

% DESCRIPTION LOGICS
%---------------------------------------------------------------
\newcommand{\shiqd}{\ensuremath{\mathcal{SHIQ}(\mathbf{D})}\xspace}

\newcommand{\shoin}{\text{$\mathcal{SHOIN}$}\xspace}
\newcommand{\shoiq}{\text{$\mathcal{SHOIQ}$}\xspace}
\newcommand{\sroiq}{\text{$\mathcal{SROIQ}$}\xspace}
\newcommand{\sroiqd}{\ensuremath{\mathcal{SROIQ}(\mathbf{D})}\xspace}
\newcommand{\KB}{\text{$\mathcal{K}$}\xspace}
%\newcommand{\ALC}{\ensuremath{\mathcal{ALC}}\xspace}

\newcommand{\ALCN}{\ensuremath{\mathcal{ALCN}}\xspace}
\newcommand{\ALCO}{\ensuremath{\mathcal{ALCO}}\xspace}

\newcommand{\DLs}{DLs\xspace}
\newcommand{\DL}{DL\xspace}
\newcommand{\dls}{description logics\xspace}
\newcommand{\dl}{description logic\xspace}

\newcommand{\ABox}{ABox\xspace}
\newcommand{\ABoxes}{ABoxes\xspace}
\newcommand{\TBox}{TBox\xspace}
\newcommand{\RBox}{RBox\xspace}

% sroiq syntax
\newcommand{\Inv}{\text{$\mathsf{Inv}$}\xspace}
%\newcommand{\Ref}{\text{$\mathsf{Ref}$}\xspace}
\newcommand{\Irr}{\text{$\mathsf{Irr}$}\xspace}
\newcommand{\Sym}{\text{$\mathsf{Sym}$}\xspace}
\newcommand{\Asy}{\text{$\mathsf{Asy}$}\xspace}
\newcommand{\Tra}{\text{$\mathsf{Tra}$}\xspace}
\newcommand{\Dis}{\text{$\mathsf{Dis}$}\xspace}
\newcommand{\Self}{\ensuremath{\mathit{Self}}}
\newcommand{\concept}[1]{\ensuremath{\mathit{#1}}\xspace}
\newcommand{\rolename}[1]{\ensuremath{\mathit{#1}}\xspace}

% vocabulary
\newcommand{\NcDL}{\text{$N_{C}$}}
\newcommand{\NrDL}{\text{$N_{R}$}}
\newcommand{\NiDL}{\text{$N_{I}$}}
\newcommand{\NvDL}{\text{$N_{V}^{dl}$}}

% cal symbols
\newcommand{\calK}{\text{$\mathcal{K}$}\xspace}
\newcommand{\calR}{\text{$\mathcal{R}$}\xspace}
\newcommand{\Rh}{\text{$\mathcal{R}_h$}\xspace}
\newcommand{\Ra}{\text{$\mathcal{R}_a$}\xspace}
\newcommand{\calT}{\text{$\mathcal{T}$}\xspace}
\newcommand{\calA}{\text{$\mathcal{A}$}\xspace}
\newcommand{\calC}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\calB}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\calD}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\calF}{\ensuremath{\mathcal{F}}\xspace}
\newcommand{\calL}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\calM}{\ensuremath{\mathcal{M}}\xspace}
\newcommand{\bfR}{\text{$\mathbf{R}$}\xspace}
\newcommand{\bfB}{\ensuremath{\mathbf{B}}\xspace}
\newcommand{\bfI}{\ensuremath{\mathbf{I}}\xspace}
\newcommand{\bfC}{\text{$\mathbf{C}$}\xspace}
% interpretations
\newcommand{\calI}{\text{$\mathcal{I}$}\xspace}
\newcommand{\calJ}{\text{$\mathcal{J}$}\xspace}

% functions
\newcommand{\extract}{\ensuremath{\mathit{extract}}\xspace}
\newcommand{\enumeration}{\ensuremath{\mathit{enumerate}}\xspace}

% normalization
\newcommand{\norm}{\ensuremath{\Omega}\xspace}
\newcommand{\nnf}{\ensuremath{\mathsf{nnf}}\xspace}
\newcommand{\pos}{\ensuremath{\mathsf{pos}}\xspace}

%\newcommand{\false}{\ensuremath{\mathsf{false}}\xspace}
%\newcommand{\true}{\ensuremath{\mathsf{true}}\xspace}

% translation
%\newcommand{\trans}{\ensuremath{\mathit{trans}}\xspace}
\newcommand{\ar}{\ensuremath{\mathit{ar}}\xspace}

% LOGIC PROGRAMS
%---------------------------------------------------------------
\newcommand{\NpLP}{\text{$N_{R}^{lp}$}}
\newcommand{\NfLP}{\text{$N_{F}^{lp}$}}
\newcommand{\NvLP}{\text{$N_{V}^{lp}$}}
\newcommand{\NcLP}{\text{$N_{C}^{lp}$}}

% Lp syntax
%\newcommand{\naf}{\texttt{$\mathsf{not}$}}
\newcommand{\Prog}{\ensuremath{\mathrm{\Pi}}\xspace}
\newcommand{\Rule}{\ensuremath{\rho}\xspace}

\newcommand{\impl}{\text{:$-$}\xspace}
\newcommand{\calP}{\text{$\mathcal{P}$}}

\newcommand{\body}[1]{B(#1)}
\newcommand{\bodyp}[1]{B^+(#1)}
\newcommand{\bodyn}[1]{B^-(#1)}
\newcommand{\BU}{{\ensuremath{B_{\cal U}}}}
\newcommand{\commadots}[0]{,\ldots ,}
\newcommand{\derives}{\la}
\newcommand{\GP}{\ensuremath{Gr(\p)}}
\newcommand{\head}[1]{H(#1)}
\newcommand{\la}{\leftarrow}
\newcommand{\naf}{{\it not}\,}
%\newcommand{\p}{\ensuremath{{\pi}}}
\newcommand{\U}{{\ensuremath{\cal U}}}
\newcommand{\UP}{\ensuremath{U_{\p}}}
% 
\newcommand{\bfT}{\text{$\mathbf{T}$}}
\newcommand{\bfTT}{\text{$\mathbf{T_T}$}}

\newcommand{\aggr}{\text{$\#aggr$}}
\newcommand{\aggrcount}{\ensuremath{\mathit{\#count}}}
\newcommand{\aggrsum}{\text{$\mathsf{\#sum}$}}
\newcommand{\aggrmax}{\text{$\mathsf{\#max}$}}
\newcommand{\aggrmin}{\text{$\mathsf{\#min}$}}

\newcommand{\thing}{\ensuremath{\concept{\top}}\xspace}

% Semantics
\newcommand{\HU}{\ensuremath{\mathcal{U}}\xspace}
\newcommand{\HB}{\ensuremath{\mathcal{B}}\xspace}

\newcommand{\grnd}{\ensuremath{\mathit{Gr}}}

% Answer Sets
\newcommand{\AS}{\mathcal{AS}}

% Tools
\newcommand{\Clingo}{\ensuremath{\mathtt{Clingo}}\xspace}
\newcommand{\Wolpert}{\ensuremath{\mathtt{Wolpertinger}}\xspace}
\newcommand{\Konclude}{\ensuremath{\mathtt{Konclude}}}
\newcommand{\HermiT}{\ensuremath{\mathtt{HermiT}}\xspace}
\newcommand{\Protege}{Prot\'eg\'e\xspace}


==> macros/mymacros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                    ** mymacros.tex **                     %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\usepackage{comment}
%\usepackage{ifpdf}

\newcommand{\skipit}[1]{} % used to skip proofs
\newcommand{\addit}[1]{} % used to skip proofs

% hs macros
% definitions
\newcommand{\define}[1]{\emph{#1}}
% math & logic
\newcommand{\N}{\mathbb{N}}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\guard}{\mathrel{\left.\middle\vert\right.}}
\newcommand{\card}[1]{\left\vert#1\right\vert}
\newcommand{\size}[1]{\left\Vert#1\right\Vert}
% prototypical quantifier
\newcommand{\Q}{\rotatebox[origin=c]{180}{\scalebox{0.90}{\raisebox{-1.6ex}[0ex][0ex]{$\mathsf{Q}$}}}}
%\newcommand{\eqdef}{\mathrel{{=\!}_{\mbox{\em\tiny def}}}}
\renewcommand{\eqdef}{\mathrel{\,:=\,}}
\newcommand{\iffdef}{\mathrel{\,:\mathrel{\mkern-6mu}{\Longleftrightarrow}\,}}
\newcommand{\ebnfeq}{\mathrel{::=}}
\newcommand{\bigland}{\bigwedge}
\newcommand{\biglor}{\bigvee}
\newcommand{\limplies}{\rightarrow}
\renewcommand{\land}{\mathrel{\wedge}}
\renewcommand{\lor}{\mathrel{\vee}}
\newcommand{\Trans}{\mathrm{Trans}}
\newcommand{\trans}{\mathrm{trans}}
\newcommand{\svec}[1]{\vec{#1}\,}
\newcommand{\pick}[1]{\mathsf{pick}\!\left(#1\right)}
% paper-specific special symbols
\newcommand{\Sub}{\mathit{Sub}}
\newcommand{\M}{\mathcal{M}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\PV}[1]{\mathcal{P}_{#1}}
\newcommand{\Pphi}{\PV{\phi}}
\newcommand{\preq}{\simeq}
% precisifications
\def\uspd{{\sim}^{-1}} % unique sim-predecessor
% signature/vocabulary of first-order logic
\def\Stands{\mathcal{S}}
\def\sts{\spform{s}} % standpoint symbol
\def\Preds{\mathcal{P}}
\def\Funcs{\mathcal{F}}
\def\Consts{\mathcal{C}}
\def\Vars{\mathcal{V}}
\def\Terms{\mathcal{T}}
\def\E{\mathcal{E}}
\def\StandExps{\E_{\Stands}}
\def\ste{\spform{e}} % standpoint expression (possibly compound)
\def\sigmaE{\sigma_{\E}}
\def\transE{\trans_{\E}}
\def\Atoms{\mathcal{A}}
\def\Formulas{\mathbb{S}}
% Kripke structures
\def\KStructs{\mathbb{M}}
\def\kstruct{\mathfrak{M}}
% first order structures
\def\Structs{\mathbb{I}}
% (ordinary) first-order structure (interpretation without variable valuation)
\def\struct{\mathcal{I}}
% variable assignment for first-order semantics
\def\varassign{v}
% interpretation function for FOL
\def\intf{\cdot^{\struct}}
% interpretation domain
\def\Dom{\Delta}
% domain element
\def\de{\delta}
% apply interpretation function to syntax element
\newcommand{\interpret}[2]{#1^{#2}}
\newcommand{\interprets}[1]{\interpret{#1}{\struct}}
\newcommand{\interpretsv}[1]{\interpret{#1}{\struct,\varassign}}
\newcommand{\interpretgp}[1]{\interpret{#1}{\gamma(\pr)}}
\newcommand{\interpretgpv}[1]{\interpret{#1}{\gamma(\pr),\varassign}}

%% languages
% description logics
\def\EL{\ensuremath{\mathcal{E\!L}}\xspace}
\def\FL{\ensuremath{\mathcal{F\!L}}\xspace}
\newcommand{\ebnfoptional}[1]{\textcolor{gray}{\;\mid #1}}

%% predicates and functions in examples
% general way of styling first-order predicates
%\newcommand{\pred}[1]{\textcolor{teal}{\mathit{#1}}}
% style function symbols likewise for now
\newcommand{\func}[1]{\textcolor{olive}{\mathit{#1}}}
% style standpoint symbols sans serif
\newcommand{\stan}[1]{\scaleobj{0.9}{\mathsf{#1}}}
% show an example formula and its intended meaning
\newcommand{\formulaexample}[2]{\item #1~\ldots~#2}
% concrete symbols
\def\lay{\stan{lay}}
\def\pro{\stan{pro}}
\def\patient{\pred{Patient}}
\def\medpro{\pred{MedicalPro}} % medical professional
\def\meddev{\pred{MedicalDevice}}
\def\expert{\pred{Expert}}
\def\hasPart{\pred{HasPart}}
\def\hasFunction{\pred{HasFunction}}
\def\infPump{\pred{InfusionPump}}
\def\pump{\func{InfP1}}
\def\onOffButton{\func{OnOffButton}}
\def\healing{\func{Healing}}
\def\power{\func{Power}}
\def\john{\func{John}}
\def\marge{\func{Margaret}}

\def\dland{\sqcap}
\def\dlor{\sqcup}
\def\dlsub{\sqsubseteq}

%% text macros
\def\FOSL{FOSL\xspace}
\def\fosl{first-or\-der stand\-point logic\xspace}
\def\FOSSs{First-Or\-der Stand\-point Structures\xspace}
\def\foss{first-or\-der stand\-point structure\xspace}
\def\fosss{first-or\-der stand\-point structures\xspace}

\def\mysubsection#1{\vskip2pt\textbf{#1}\\[1pt]}

\newcommand{\tad}{\hspace{1pt}}

% manually define proof environment for LNCS
\newenvironment{proof}{\paragraph{Proof.}}{\hfill\qed}
\newenvironment{claimproof}{\paragraph{Proof (of the claim):}}{\hfill\textit{(This proves the claim.)}}


\newenvironment{narrowalign}{\\[3pt]\mbox{}\hfill}{\hfill\mbox{}\\[4pt]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  END END END         (of mymacros.tex)      END END END   %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> macros/preamble.tex <==
% Use the postscript times font!
\usepackage{times}
\usepackage{soul}
\usepackage{url}
\usepackage[hidelinks]{hyperref}
\usepackage[utf8]{inputenc}
\usepackage[small]{caption}
\usepackage{graphicx}
\usepackage{amsmath}
%\usepackage{amsthm}
\usepackage{booktabs}
\usepackage{algorithm}
\usepackage{algorithmic}
\urlstyle{same}
\renewcommand*\ttdefault{txtt}


\usepackage[british]{babel}
\usepackage[usenames,x11names]{xcolor}
\usepackage{relsize,setspace}
\usepackage{stmaryrd}
\usepackage[font=it]{caption}
\usepackage{tikz,pgf}\usetikzlibrary{shapes,backgrounds}

\usepackage{amssymb}
\usepackage{pifont}

%%%% Alternative symbol
%\usepackage[amsthm,thref,thmmarks]{ntheorem}
%\renewcommand{\proofSymbol}{\ensuremath{\mbox{\ding{113}}}}

%\usepackage[pdftex,colorlinks=true,linkcolor=black,citecolor=black,menucolor=black,urlcolor=black]{hyperref}
\usepackage{cleveref}  % allows to ref without putting the environment name
% i.e. write "\Cref(ex)" instead of "Example \ref{ex}"

\usepackage{multirow}
\usepackage{comment}
\usepackage{xspace}
\usepackage{pdflscape}
\usepackage{yhmath}

\usepackage[inline]{enumitem}

%\usepackage{enumitem}
\setlist{leftmargin=*,noitemsep,parsep=0.2ex,topsep=0.3ex}
%\setlist[itemize]{noitemsep,parsep=0.2ex,topsep=0.3ex}
%\setlist[enumerate]{noitemsep,parsep=0.2ex,topsep=0.3ex}
\setlength{\jot}{2pt}
\usepackage{scalerel}

\usepackage{microtype}


%\newcommand{\shadydiamond}{\mbox{{\rotatebox[origin=c]{45}{\small\ding{113}}}}}

% environments
%\theoremstyle{plain}
%\theoremseparator{.}
%\theoremheaderfont{\normalfont\bfseries}
%\theorembodyfont{\slshape}
%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{observation}[theorem]{Observation}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{conjecture}[theorem]{Conjecture}
%\theorembodyfont{\upshape}
%\theoremsymbol{\ensuremath{\shadydiamond}}
%\newtheorem{definition}{Definition}
%\newtheorem{example}{Example}
%\theoremheaderfont{\normalfont\bfseries}
%\theorembodyfont{\slshape}
%\newtheorem{claim}{Claim}
%\newtheorem{nonumberlemma}{Lemma}
%\newtheorem{nonumbertheorem}{Theorem}
%\theoremheaderfont{\normalfont\itshape}
%\theoremsymbol{\ensuremath{\Box}}
%\newtheorem{proof}{Proof}
%\newtheorem{proofsketch}{Proof sketch} % note that this does not care \iflong
% this is for nesting proofs, e.g. proving some distinguished sub-claim within a proof
%\theoremstyle{nonumberplain}
%\theoremheaderfont{\normalfont\itshape}
%\theoremsymbol{\ensuremath{\shadydiamond}}
%\newtheorem{claimproof}{Proof of the claim}

% %% for producing a long version of the paper with proofs
\usepackage{ifthen}
% \usepackage{environ}
% %% this could in principle be used to use “long” and “short” as non-exclusive or non-exhaustive, or both
% %\newif\ifshort
\newif\iflong
\longfalse
% % use shortproofs for proofs that should appear in the short paper, but not in the long paper
% \NewEnviron{shortproof}{\iflong\else\expandafter\begin{proof}\BODY\end{proof}\fi}
% % shortproofsketches are a variant (special case) of short proofs where the environment says “Proof sketch” instead of “Proof”
% \NewEnviron{shortproofsketch}{\iflong\else\expandafter\begin{proofsketch}\BODY\end{proofsketch}\fi}
% % use longproofs for proofs that should appear in the long paper only (i.e. not in the short paper)
% \NewEnviron{longproof}{\iflong\expandafter\begin{proof}\BODY\end{proof}\fi}

\usepackage{todonotes}

\input{macros/davidMacros}
\input{macros/ThesisSymbols}
\input{macros/mymacros}
\input{macros/dlmacros}



\def\lg#1{\textcolor{blue}{#1}} % Lucia adding comments in blue
\def\alert#1{\textcolor{red}{#1}} % Lucia adding comments in blue

